Pattern matching under DTW distance

In this work, we consider the problem of pattern matching under the dynamic time warping (DTW) distance motivated by potential applications in the analysis of biological data produced by the third generation sequencing. To measure the DTW distance between two strings, one must "warp" them, that is, double some letters in the strings to obtain two equal-lengths strings, and then sum the distances between the letters in the corresponding positions. When the distances between letters are integers, we show that for a pattern P with m runs and a text T with n runs: 1. There is an O(m + n)-time algorithm that computes all locations where the DTW distance from P to T is at most 1; 2. There is an O(kmn)-time algorithm that computes all locations where the DTW distance from P to T is at most k. As a corollary of the second result, we also derive an approximation algorithm for general metrics on the alphabet.

==> border.tex <==
\begin{lemma}\label{lm:border}
For a block $D[i_p \dd j_p, i_t \dd j_t]$ let $h=j_p-i_p$, $w =j_t-i_t$, and $d=d(P[i],T[j])$. We have for every $i_p < x \leq j_p$:
\begin{equation}\label{eq:border-right}
D[x,j_t]= \begin{cases}
D[i_p,j_t-(x-i_p)]+(x-i_p) \times d \text{ if } x-i_p \leq w; \\
D[x-w,i_t]+w \times d \text{ otherwise}.
\end{cases}
\end{equation}
For every $i_t < y \leq j_t$:
\begin{equation}\label{eq:border-bottom}
D[j_p,y]= \begin{cases}
D[j_p-(y-i_t),i_t]+(y-i_t) \times d \text{ if }  y-i_t \leq h; \\
D[i_p,y-h]+h \times d \text{ otherwise}.
\end{cases}
\end{equation}

\end{lemma}
\begin{proof}
For a homogeneous block, we have $d=0$, and we already proved in Corollary~\ref{cor:homogeneous} that all the values in such a block are equal, and the claim of the lemma is trivially true as well. We now assume $d > 0$.

Let $x$ be such that $i_p < x \leq j_p$. Let $\pi$ be a warping path realizing $D[x,j_t]$.
%
Let $(a,b)$ be the first node of $\pi$ belonging to the block.
We have $a \in [i_p,j_p]$ and $b \in [i_t,j_t]$ and either $a=i_p$ or $b=i_t$.
%
The number of edges of $\pi$ in the block from $(a,b)$ to $(x,j_t)$ must be minimal, else there would be a shorter path, thus it is equal to $\max(x-a,j_t-b)$ and: 
$$D[x,j_t]=D[a,b]+\max(x-a,j_t-b)\times d$$
We divide the analysis in cases which are illustrated in Figure~\ref{fig:border}.

\noindent
\underline{Case 1: $x-i_p \leq w$.} Consider the cell $(i_p,j_t - (x-i_p))$. There is a path from $(i_p,j_t - (x-i_p))$ to $(x,j_t)$ that takes $x-i_p$ diagonal steps inside the block, and therefore $D[x,j_t] \leq D[i_p,j_t - (x-i_p)]+(x-i_p)\times d$. We now show that $D[x,j_t] \geq D[i_p,j_t - (x-i_p)]+(x-i_p)\times d$, which implies the claim of the lemma.
\begin{enumerate}[label=(\alph*)]
\item If \underline{$a=i_p$ and $b \geq j_t - (x-i_p)$}, then $\max(x-i_p,j_t-b)=x-i_p$. We have:
\begin{align*}
D[x,j_t]&=D[i_p,b]+(x-i_p)\times d \\
& \geq D[i_p,j_t - (x-i_p)]+(x-i_p)\times d \text{ (via Lemma~\ref{lm:non-decreasing})}
\end{align*}
\item If \underline{$a=i_p$ and $b < j_t - (x-i_p)$}, then $\max(x-i_p,j_t-b)=j_t-b$. As there is a path from $(a,b) = (i_p,b)$ to $(i_p,j_t - (x-i_p))$ of length $(j_t - (x-i_p)-b)$, we have $D[i_p,j_t - (x-i_p)] \le D[i_p,b] + (j_t - (x-i_p)-b) \times d$. Consequently,
\begin{align*}
D[x,j_t]&=D[i_p,b]+(j_t-b)\times d\\
& \geq D[i_p,j_t - (x-i_p)] - (j_t - (x-i_p)-b) \times d +(j_t-b) \times d \text{ (via Claim~\ref{claim:recursion})}\\
& \geq D[i_p,j_t - (x-i_p)]+(x-i_p)\times d
\end{align*}
\item If \underline{$b=i_t$}, then $i_p \leq a$ and $\max(x-a, j_t-b) \leq \max(x-i_p,w) = w$. As there is a path from $(i_p,i_t)$ to $(i_p,j_t - (x-i_p))$ of length $(j_t - (x-i_p)-i_t)$, we have $D[i_p,j_t - (x-i_p)] \le D[i_p,i_t] + (j_t - (x-i_p)-i_t) \times d$. Therefore, 
\begin{align*}
D[x,j_t]&=D[a,i_t]+w\times d\\
& \geq D[i_p,i_t] +w\times d \text{ (via Lemma~\ref{lm:non-decreasing})} \\
& \geq D[i_p,j_t - (x-i_p)] - (j_t - (x-i_p)-i_t) \times d +w\times d\\
& \geq D[i_p,j_t - (x-i_p)]+(x-i_p)\times d
\end{align*}
\end{enumerate}

\noindent
\underline{Case 2: $x-i_p > w$.} Consider a cell $(x-w,i_t)$. There is a path from $(x-w,i_t)$ to $(x,j_t)$ that takes $w$ diagonal steps inside the block, and therefore $D[x,j_t] \leq D[x-w,i_t]+l\times d$. We now show that $D[x,j_t] \geq D[x-w,i_t]+w\times d$, which implies the claim of the lemma.
\begin{enumerate}

\item If \underline{$b=i_t$ and $a \ge x-w$},
then $\max(x-a,j_t-b) = \max(x-a,w)=w$ and we have:
\begin{align*}
D[x,j_t]&=D[a,i_t]+w\times d \\
& \geq D[x-w,i_t] +w\times d \text{ (via Lemma~\ref{lm:non-decreasing})} 
\end{align*}

\item  If \underline{$b=i_t$ and $a < x-w$}, then $\max(x-a,j_t-b)= \max(x-a,w)=x-a$. As there is a path from $(a,i_t)$ to $(x-w,i_t)$ of length $(x-w-a)$, we have $D[x-w,i_t] \leq D[a,i_t] + (x-w-a) \times d$ by definition. Therefore, 
\begin{align*}
D[x,j_t]&=D[a,i_t]+(x-a)\times d\\
& \geq D[x-w,i_t] - (x-w-a) \times d+(x-a) \times d\\
& \geq D[x-w,i_t] + w\times d
\end{align*}
%
\item If \underline{$a=i_p$}, 
$b \geq i_t$ and thus $\max(x-a,j_t-b) \leq \max(x-i_p,w) = x-i_p$. Additionally, as there is a path from $(i_p,i_t)$ to $(x-w,i_t)$ of length $(x-w - i_p)$ we have $D[x-w,i_t] \le D[i_p,i_t] + (x-w-i_p) \times d$. Consequently,
\begin{align*}
D[x,j_t]&=D[i_p,b]+(x-i_p)\times d \\
& \geq D[i_p,i_t] +(x-i_p)\times d \text{ (via Lemma~\ref{lm:non-decreasing})} \\
& \geq D[x-w,i_t] - (x-w-i_p) \times d +(x-i_p)\times d\\
& \geq D[x-w,i_t] + w\times d
\end{align*}
\end{enumerate}

Note that the proof uses two facts: the fact that $D[i,j]$ is the minimal cost of a warping path that starts in row zero and Lemma~\ref{lm:non-decreasing}). Both facts are symmetric for $x$ and $y$, and therefore the proof of the claim of the lemma for every $i_t < y \leq j_t$ can be shown analogously.

\end{proof}

\input{lem7}


==> lce.tex <==
In this section, we show Lemma~\ref{lm:1-DTW} that for a pattern $P$ with $m$ runs and and text $T$ with $n$ runs gives an $\Oh(m+n)$-time algorithm.  

\begin{definition}[RLE-diagonals]
We say that a sequence of blocks forms an \emph{RLE-diagonal} if the blocks are formed by runs $i, i+1, \ldots, j$ of $P$ and $i+\delta, i+1+\delta, \ldots, j+\delta$ of $T$, for some integers $i,j,\delta$. 
\end{definition}

\begin{definition}[Streak]
A $q$-streak is a maximal subsequence of an RLE-diagonal containing sequential homogeneous $q$-blocks. 
\end{definition}

\begin{observation}\label{obs:zero_streak}
If $D[i,j] = 0$, then it belongs to a $0$-streak. Furthermore, each $0$-streak necessarily starts in the first row of $D$.
\end{observation}
\begin{proof}
By definition, there must be a path from the first row of $D$ to $D[i,j]$ containing $0$-values only. For every $0$-value $D[i',j']$ we must have $P[i'] = T[j']$, and therefore every such value must belong to a homogeneous $0$-block. Furthermore, two homogeneous blocks can only be neighbours diagonally, else it would contradict the maximality of the runs. The claim follows. 
\qed
\end{proof}

\begin{observation}\label{obs:one_value}
If $D[i,j] = 1$, then $D[i,j]$ belongs to a $1$-streak or neighbours a block in a $0$-streak.
\end{observation}
\begin{proof}
If $P[i]=T[j]$, we are in a homogeneous block and $D[i,j]$ belongs to a $1$-streak, and we are done. Otherwise, we have $P[i] \neq T[j]$ and there is a path $(i_1,j_1), (i_2,j_2), \ldots, (i_q,j_q)$ such that $i_1 = 1$, $(i_q,j_q) = (i,j)$, and $D[i_{q},j_{q}] = \sum_{q'=1}^{q} d(P[i_{q'}], T[j_{q'}])$. It follows that for all $1 \le q' \le q-1$, $d(P[i_{q'}], T[j_{q'}]) = 0$, and therefore $D[i_{q'}, j_{q'}]$ must belong to a $0$-streak by Observation~\ref{obs:zero_streak}. 
\qed
\end{proof}
 

\repeatlemma{1DTW}
\begin{proof}
For a string $S$, define $\overline{RLE}(S)$ to be a string such that $\overline{RLE}(S)[i]$ contains the letter forming the $i$-th run of $S$. We preprocess $P' = \overline{\RLE}(P)$ and $T' = \overline{\RLE}(T)$ in $\Oh(m+n)$ time and space to maintain longest common suffix queries in constant time~\cite{RMQ}. The input of a longest common suffix query are two positions $i,j$ of $P'$ and $T'$ respectively, and the output is the largest $\ell$ such that $P'[i-\ell \dd i] = T'[j-\ell \dd j]$.

Let $B_i$, $1 \le i \le n$, be the block of $D$ formed by the $m$-th run in $P$ and the $i$-th run in $T$. Using one longest common suffix query for each block $B_i$, we find the maximal streak containing it. If this streak reaches the first row of $D$, it is a $0$-streak and we can fill the last row of $B_i$ with zeros. 

We must now decide which entries in the $M$-th row of $D$ must be filled with one. Consider an entry $D[M,\ell] \neq 0$ that belongs to a block $B_i$. 

If $B_i$ is contained in a streak of length at least one, then for $D[M,\ell]$ to be equal to one, it must be a $1$-streak. Consider the first block in the maximal  streak containing $B_i$, and let $c$ be the cell in its top left corner. Because $c$ can not be equal to zero, it suffices to check whether the value in $c$ equals one. Consider a path realizing the value of $c$. It goes either through the left neighbour $\ell$ of $c$, the top neighbour $t$ of $c$, or the diagonal neighbour $d$ of $c$. Furthermore, the value in $c$ equals the minimum of the values in $\ell, d, t$, and therefore, at least one of these values equals one, and neither of them can belong to a $1$-streak. By Observation~\ref{obs:one_value}, such a cell must neighbour a block in a zero-streak. For each block neighbouring the cells $\ell, d, t$, we use one longest common suffix query to decide whether they are contained in a $0$-streak. If they are, then the value in $c$, and consequently all the values in $B_i$, including the values in the last row of $B_i$, are equal to one, and we fill them in appropriately. 

Suppose now that $B_i$ does not belong to a streak. For $D[M,\ell]$ to be equal to one, it must neighbour a block in a $0$-streak. Therefore, there can be only one such cell in $B_i$, the one in the left bottom corner, and we can decide whether the value in it equals to one in constant time similar to above. 
\qed
\end{proof}
